Radio Detection of 18 Rass BL Lac Objects

We present the radio detection of 18 BL Lac objects from our survey of over 575 square degrees of sky. These 18 objects are located within 20 arcsec of the X-ray position, of which 11 have a measured red-shift. All candidates are radio emitters above ~1 mJy and fall within the range of existing samples on the two colour, alpha_ro vs alpha_ox, diagram with a transitional population of three (3) evident. Two unusual sources have been identified, a candidate radio quiet BL Lac, RX J0140.9-4130, and an extreme HBL, RX J0109.9-4020, with Log(nu_peak)~19.2. The BL Lac Log(N)-Log(S) relation is consistent with other samples and indicates the ROSAT All Sky Survey (RASS) could contain (2000+-400) BL Lac objects.

==> astro.tex <==
\def\tg{\mathop{\rm tg}\nolimits}
\def\arctg{\mathop{\rm arctg}\nolimits}

\def\point#1{\hbox{\setbox7=\hbox to0.8em{\hfil.\hfil}%
\setbox8=\hbox to0.8em{\hfil$^{#1}$\hfil}%
\box7\kern-0.8em\box8}}

\def\dd{\point{\rm d}}
\def\hh{\point{\rm h}}
\def\mm{\point{\rm m}}
\def\ss{\point{\rm s}}

\def\oo{\point{\circ}}
\def\ll{\point{\prime}}
\def\uu{\point{\prime\prime}}




==> bull-zag.tex <==
\magnification=\magstep0
\baselineskip=3.1truemm 
\vsize=230truemm 
\hsize=165truemm 
\parindent=1truecm
\parskip=0pt plus2truept 

\def\nav{\leavevmode\lower.5em\hbox{"}} 

\def\hang{\hangindent\parindent}
\def\item{\par\hang\textindent}
\def\itemitem{\par\indent \hangindent2\parindent \textindent}
\def\textindent#1{\indent\llap{#1\enspace}\ignorespaces}

\catcode`@=11

\newdimen\pagewidth \newdimen\pageheight \newdimen\ruleht
  \maxdepth=2.2pt  \parindent=.5truecm
\pagewidth=\hsize  \pageheight=\vsize  \ruleht=.5pt
\abovedisplayskip=6pt plus 3pt minus 1pt
\belowdisplayskip=6pt plus 3pt minus 1pt
\abovedisplayshortskip=0pt plus 3pt 
\belowdisplayshortskip=4pt plus 3pt 

\newinsert\margin
\dimen\margin=\maxdimen
\count\margin=0 \skip\margin=0pt

\def\footnote#1{\edef\@sf{\spacefactor\the\spacefactor}#1\@sf
     \insert\footins\bgroup\eightrm
     \insertlinepenalty100 \let\par=\endgraf
       \leftskip=0pt \rightskip=0pt
       \splittopskip=10pt plus 1pt minus 1pt \floatingpenalty20000
       \smallskip\item{#1}\bgroup\strut\aftergroup\@foot\let\next}
\skip\footins=12pt plus 2pt minus 4pt
\dimen\footins=.6truecm
\newif\iftitle
\def\titlepage{\global\titletrue}

\def\headl{\vbox to 1cm{{\ifodd\pageno\rightheadline \else 
\leftheadline\fi}\vskip1mm\hrule}} 
\def\headr{\vbox to 1cm{}}
\headline={\ifnum\pageno=\ppp \vbox{\headr} \else \vbox{\headl} \fi}  

\def\rightheadline{\hbox to \pagewidth{\centerline{\rhead}}} 
\def\leftheadline{\hbox to \pagewidth{\centerline{\lhead}}}

\def\makefootline{\baselineskip=2truecc \line{\the\footline}}
  \def\nonumbers{\hbox to \pagewidth{
                 \vbox to 6mm{}
                 \hfill}}
\footline{\ifodd\pageno\rightfootline
          \else\leftfootline\fi}
  \def\rightfootline{\hbox to \pagewidth{
                     \vbox to 6mm{}
                     \hfill\tenrm\folio}}
  \def\leftfootline{\hbox to \pagewidth{
                     \vbox to 6mm{}
                     \tenrm\kern-8pt\folio\hfill}}

\def\onepageout#1{\shipout\vbox{
  \offinterlineskip
\vbox to 1cm{\ifnum\pageno=\ppp \vbox{\headr} \else 
\vbox{\headl} \fi}
  \vbox to \pageheight{
    \ifvoid\margin\else
     \rlap{\kern31cc\vbox to0pt{\kern4pt\box\margin \vss}}\fi
    #1
    \ifvoid\footins\else
     \vskip\skip\footins \kern-3pt
     \hrule height\ruleht width 4cm \kern-\ruleht \kern3pt
     \unvbox\footins\fi
    \boxmaxdepth=\maxdepth}
  \vbox to \pageheight{
     \ifnum\pageno<500     
     {\ifodd\pageno\rightfootline\else\leftfootline\fi} 
     \else\nonumbers\fi}}
\advancepageno}
               
\def\setcornerrules{\hbox to \pagewidth{
    \vrule width 1cc height\ruleht \hfil \vrule width 1cc}
  \hbox to \pagewidth{\llap{\sevenrm(page \folio)\kern1cc}
    \vrule height1cc width\ruleht depth0pt
    \hfil \vrule width\ruleht depth0pt}}
\output{\onepageout{\unvbox255}}
 
\newbox\partialpage

\def\dvekolone{\begingroup
  \output={\global\setbox\partialpage=\vbox{\unvbox255}}\eject
  \output={\doublecolumnout} \hsize=80mm \vsize=460mm}
 
\def\krajdvekolone{\output={\balancecolumns}\eject
  \endgroup \pagegoal=\vsize}

\def\doublecolumnout{\splittopskip=\topskip \splitmaxdepth=\maxdepth
  \dimen@=230mm \advance\dimen@ by-\ht\partialpage
  \setbox0=\vsplit255 to\dimen@ \setbox2=\vsplit255 to\dimen@
  \onepageout\pagesofar \unvbox255 \penalty\outputpenalty}

\def\pagesofar{\unvbox\partialpage
  \wd0=\hsize \wd2=\hsize \hbox to\pagewidth{\box0\hfil\box2}}

\def\balancecolumns{\setbox0=\vbox{\unvbox255} \dimen@=\ht0
  \advance\dimen@ by\topskip \advance\dimen@ by-\baselineskip
  \divide\dimen@ by2 \splittopskip=\topskip
  {\vbadness=10000 \loop \global\setbox3=\copy0
    \global\setbox1=\vsplit3 to\dimen@
    \ifdim\ht3>\dimen@ \global\advance\dimen@ by1pt \repeat}
  \setbox0=\vbox to\dimen@{\unvbox1} \setbox2=\vbox to\dimen@{\unvbox3}
  \pagesofar}

\def\cstok#1{\leavevmode\thinspace\hbox{\vrule\vtop{\vbox{\hrule\kern3pt
             \hbox{\vphantom\thinspace{#1}\thinspace}}
             \kern3pt\hrule}\vrule}\thinspace}    

\def\okvir#1{\vbox{\hrule\hbox{\vrule\kern0mm
             \vbox{\kern3mm#1\kern3mm}\kern0mm\vrule}\hrule}}

\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern1mm
             \vbox{\kern1mm#1\kern1mm}\kern1mm\vrule}\hrule}}


\def\leftdisplay#1$${\leftline{\indent$\displaystyle{#1}$}$$}

\def\br{\break}%

\voffset=-.3cm
%\hoffset=.3cm
\hoffset=-.2cm






==> mjyu.tex <==
\def\nava{\leavevmode\hbox{,\kern-0.09em,}}%yu-navodnik-pocetni
\def\navb{\char'134}                                      %yu-navodnik-krajnji
\def\DJ{\leavevmode\setbox0=\hbox{D}\kern0pt
 \rlap{\kern.04em\raise.188\ht0\hbox{-}}D}
\def\dj{\leavevmode\setbox0=\hbox{d}\kern0pt
 \rlap{\kern.215em\raise.46\ht0\hbox{-}}d}
\def\SH{\v S} \def\sh{\v s} % Sasinci
\def\CJ{\' C} \def\cj{\' c} % Cicevac
\def\CH{\v C} \def\ch{\v c} % Xaxak
\def\Z{\v Z} \def\z{\v z} % Zuzemberk
\def\br{\break}



==> wncyr.tex <==
\def\rrmd{\font\tipo=wncyr12\tip}%
\def\rbfd{\font\tipo=wncyb12\tip}%
\def\rssd{\font\tipo=wncyss12\tip}%
\def\rrm{\font\tipo=wncyr10\tip}%
\def\rbf{\font\tipo=wncyb10\tip}%
\def\rit{\font\tipo=wncyi10\tip}%
\def\rss{\font\tipo=wncyss10\tip}%
\def\rsc{\font\tipo=wncysc10\tip}%
\def\rrmdev{\font\tipo=wncyr9\tip}%
\def\rbfdev{\font\tipo=wncyb9\tip}%
\def\ritdev{\font\tipo=wncyi9\tip}%
\def\rssdev{\font\tipo=wncyss9\tip}%
\def\rrmos{\font\tipo=wncyr8\tip}%
\def\rbfos{\font\tipo=wncyb8\tip}%
\def\ritos{\font\tipo=wncyi8\tip}%
\def\rssos{\font\tipo=wncyss8\tip}%
\def\rrmsev{\font\tipo=wncyr7\tip}%
\def\rbfsev{\font\tipo=wncyb7\tip}%
\def\ritsev{\font\tipo=wncyi7\tip}%
\def\tip{\relax\tipo\def\DD{\tipo\char'006}\def\dd{\tipo\char'016}% \tip
\def\DJ{\DD}\def\dj{\dd}% 
\def\ZZ{\tipo\char'021}\def\zz{\tipo\char'031}%
\def\Z{\ZZ}\def\z{\zz}%
\def\LJ{\tipo\char'001}\def\lj{\tipo\char'011}%
\def\NJ{\tipo\char'000}\def\nj{\tipo\char'010}%
\def\CC{\tipo\char'007}\def\cc{\tipo\char'017}%
\def\DZ{\tipo\char'002}\def\dz{\tipo\char'012}%
\def\XX{Q}\def\xx{q}%
\def\JJ{J}\def\jj{j}% 
\def\SS{X}\def\ss{x}%
\def\JA{\tipo\char'027}\def\ja{\tipo\char'037}%
\def\SC{W}\def\sc{w}%
\def\CJ{\CC}\def\cj{\cc}%
\def\CH{Q}\def\ch{q}%
\def\SH{X}\def\sh{x}%
% sch="x"; tvrdo i = "y"; ja = "j"; schtsch = "w"; tsch = "q"
\def\EE{\tipo\char'003}\def\ee{\tipo\char'013}% "e oborotnoe"
\def\JI{\tipo\char'022}\def\ji{\tipo\char'032}% rusko "j"
\def\JU{\tipo\char'020}\def\ju{\tipo\char'030}%
\def\M{\tipo\char'136}\def\m{\tipo\char'176}% meki znak
\def\TV{\tipo\char'137}\def\tv{\tipo\char'177}% tvrdi znak
\def\rnava{\tipo\char'074}\def\rnavb{\tipo\char'076}% ruski navodnici
\def\snava{\leavevmode\hbox{,\kern-0.06em,}}% yu-
\def\snavb{\tipo\char'134}}% navodnici
\def\br{\break}%



